DyFormer: A Scalable Dynamic Graph Transformer with Provable Benefits on Generalization Ability

Transformers have achieved great success in several domains, including Natural Language Processing and Computer Vision. However, its application to real-world graphs is less explored, mainly due to its high computation cost and its poor generalizability caused by the lack of enough training data in the graph domain. To fill in this gap, we propose a scalable Transformer-like dynamic graph learning method named Dynamic Graph Transformer (DyFormer) with spatial-temporal encoding to effectively learn graph topology and capture implicit links. To achieve efficient and scalable training, we propose temporal-union graph structure and its associated subgraph-based node sampling strategy. To improve the generalization ability, we introduce two complementary self-supervised pre-training tasks and show that jointly optimizing the two pre-training tasks results in a smaller Bayesian error rate via an information-theoretic analysis. Extensive experiments on the real-world datasets illustrate that DyFormer achieves a consistent 1%-3% AUC gain (averaged over all time steps) compared with baselines on all benchmarks.

==> sections/experiment_config.tex <==
\section{Experiment configuration}

==> sections/expressive_linear_gnn.tex <==
\weilin{Make some changes to construct the story:
(1) for each node, we use its induced k-hop subgraph to compute its node representation. (2) After mean-square error closed-form solution, we can use a boosting type of method to approximate the weight for cross-entropy loss. since we already have the inverse of correlation matrix, the computation cost can be very low. (3) try to argue the multi-layer non-linear gnn is not a must if we can do some feature engineering to generate some good features. try to use some expressive power analysis here. (4) another potential method is to use graph kernel regression when graph is not separable (add this as a subsection/extension)}

\weilin{there are two direction we can push in addition to this quick parameter update (another contribution): expressive power. I am checking papers to see what we can add}

Using the linear GNN as defined in Eq.~\ref{eq:feat_mat_define} have limitations: suppose we want to remove a node in graph, we can only remove its feature but cannot update its associated graph propagation matrix. Because if we update the propagation matrix (e.g., re-normalize the propagation matrix), then the affected node will be twice exponentially larger. Suppose degree is $D$ and GNN has $K$-layers. Then the number of affected nodes after removing 1 node is $D^K$. However, if we normalize the propagation matrix, the affected node will be $D^{2K}$, which can significantly enlarge the computation cost of \our.  

To reduce its impact, we propose to sample the $K$-hop subgraph of each node and compute the representation of the node based on the sampled $K$-hop subgraph.

\weilin{Q: Why we need expressive Linear GNN? A: As shown by~\cite{cong2021provable,li2018deeper}, applying multiple propagation matrices without weight matrices and non-linear activation function suffer from over-smoothing more than ordinary GNN structure, therefore making sure Linear GNN model has higher expressive power is very important.}

The $K$-hop subgraph for each node is defined as
\begin{equation}
    \mathcal{G}_i^K = (\mathcal{V}_i^K, \mathcal{E}_i^K),
\end{equation}
where $\mathcal{V}_i^K = \{v_j~|~\text{SPD}(v_i, v_j) \leq K,~\forall v_j\in\mathcal{V}\}$ and $\mathcal{E}_i^K = \{e_{j,k}~|~ e_{j,k} \in \mathcal{E}, \forall v_j,v_k \in \mathcal{V}_i^K\}$.
Then, each node is assigned with an extra feature as its shortest path distance to the center node.

\textbf{Challenges:} 
existing methods on the provable expressive GNN are relying on the uniform approximation of MLP and the injectiveness of the aggregation function, which is infeasible in Linear GNN.

\begin{theorem} [\oure-exp is at least as expressive as 1-WL and 2-WL test]
(1) if $\mathcal{G}_i^K \not\simeq \mathcal{G}_j^K$ and 1-WL test return $\text{1-WL}(\mathcal{G}_i^K) \neq \text{1-WL}(\mathcal{G}_j^K)$, then $\text{GER}(\mathcal{G}_i^K) \neq \text{GER}(\mathcal{G}_j^K)$;
(2) if if $\mathcal{G}_i^K \simeq \mathcal{G}_j^K$ 1-WL test return $\text{1-WL}(\mathcal{G}_i^K) = \text{1-WL}(\mathcal{G}_j^K)$, then $\text{GER}(\mathcal{G}_i^K) =\text{GER}(\mathcal{G}_j^K)$.
\end{theorem}

\begin{theorem} [\oure-exp can distinguish regular graphs that 1-WL and 2-WL test cannot]

\end{theorem}

==> sections/preliminary.tex <==
% \subsection{Graph Neural Network}

\paragraph{Setup.~}
In this paper, we consider semi-supervised node classification problem, where a graph $\mathcal{G}(\mathcal{V},\mathcal{E})$ with $N=|\mathcal{V}|$ nodes is given, in which each node $v_i \in \mathcal{V}$ is associated with a node feature vector $\mathbf{h}_i^{(0)} \in \mathbb{R}^{d_0}$, and only a subset of nodes $\mathcal{V}_\text{train} \subset \mathcal{V}$ are labeled. Let $\mathbf{A}, \mathbf{D} \in \mathbb{R}^{N\times N}$ denote the adjacency matrix and its associated degree matrix with $D_{i,i}=\deg(v_i)$ and $D_{i,j}=0$ if $i\neq j$. Then, the symmetric normalized propagation matrix is defined as $\mathbf{P}_\text{sym} = \mathbf{D}^{-1/2}\mathbf{A}\mathbf{D}^{-1/2}$ and the row normalized matrix is defined as $\mathbf{P}_\text{row} = \mathbf{D}^{-1}\mathbf{A}$. 

\paragraph{Graph neural networks.~}
\weilin{the content of this paragraph might be adjusted according to how Section 5 is written/empirical performance.}
We consider graph convolutional network with jumping knowledge~\cite{xu2018representation} with two different types of message passing.
The Graph Convolutional Netork (GCN) proposed in~\cite{kipf2016semi} is defined as
\begin{equation}\label{eq:semi_gcn}
    \mathbf{H}^{(\ell)} = \sigma\Big( \mathbf{P}_\text{sym} \mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)}\Big),
\end{equation}
and the GraphSAGE proposed in~\cite{hamilton2017inductive} is defined as
\begin{equation}\label{eq:graphsage}
    \mathbf{H}^{(\ell)} = \sigma\Big( \mathbf{P}_\text{row} \mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)}_1 + \mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)}_2 \Big),
\end{equation}
where $\sigma(\cdot)$ is non-linear activation function, $\mathbf{h}_i^{(\ell)} \in \mathbb{R}^{d_\ell}$ denotes the hidden representation of node $v_i$ at the $\ell$th layer.
Then, a classifier parameterized by $\mathbf{W}^{(L+1)}\in\mathbb{R}^{(d_0+d_1+\ldots+d_L)\times d_y}$ is applied to the concatenation of the node hidden representation of each layer $\mathbf{X} = [\mathbf{H}^{(0)}~|~\mathbf{H}^{(1)}~|~\ldots~|~\mathbf{H}^{(L)}]$ for prediction.
Our goal is to find a set of parameters $\bm{\theta}=\{\mathbf{W}^{(\ell)}\}_{\ell=1}^{L+1}$ by minimizing the empirical loss
\begin{equation}\label{eq:objective_func}
    \mathcal{L}(\bm{\theta}) = \frac{1}{|\mathcal{V}_\text{train}|}\sum_{v_i \in \mathcal{V}_\text{train}} \text{loss}(\hat{\mathbf{y}}_i, \mathbf{y}_i),~
    \hat{\mathbf{Y}} = \mathbf{X} \mathbf{W}^{(L+1)},~
\end{equation}
where $\text{loss}(\cdot, \cdot)$ is the loss function and $\mathbf{y}_i \in \{0,1\}^{d_y}$ is the target label of node $v_i$. 


==> sections/tables/ablation_study_in_one_table.tex <==
\begin{table}[h]
\centering
\scalebox{0.85}{
\begin{tabular}{llcccc}
\hline\hline
\textbf{Method}                    & \textbf{Metric}    &  \textbf{UCI}       & \textbf{Yelp}       & \textbf{ML-10M} \\ \hline\hline
\multirow{2}{*}{($1$) Single-tower / Full attention / With encoding} 
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   & $88.91\pm0.68$      & $73.90\pm0.21$      & $95.49\pm0.57$  \\ \hline
\multirow{2}{*}{($2$) Two-tower / Full attention / With encoding}
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   & $\bm{88.95\pm0.40}$ & $\bm{74.40\pm0.24}$ & $\bm{96.16\pm0.22}$  \\ \hline\hline
\multirow{2}{*}{($3$) Single-tower / $1$-hop neighbor / With encoding} 
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   & $85.10\pm0.15$      & $71.45\pm0.45$      & $92.18\pm0.44$  \\ \hline
\multirow{2}{*}{($4$) Single-tower / $3$-hop neighbor / With encoding}  
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   & $87.48\pm0.88$     & $72.31\pm0.22$      & $92.33\pm0.82$  \\ \hline\hline      
\multirow{2}{*}{($5$) Two-tower / Full-attention / Without encoding} 
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   & $87.87\pm0.47$      & $73.80\pm0.38$      & $92.59\pm0.35$  \\ \hline
\multirow{2}{*}{($6$) Two-tower / Full-attention / Only temporal connective encoding}
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   &                     &                     &                 \\ \hline
\multirow{2}{*}{($7$) Two-tower / Full-attention / Only Spatial distance encoding}
                                  & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
                                  & \text{Macro-AUC}   &                     &                     &                 \\ \hline
                                  \hline
\end{tabular}
}
\caption{Comparison of the \textit{Micro}- and \textit{Macro}-\textit{AUC} of ``\textit{single-tower}'' and ``\textit{two-tower}'', ``\textit{full attention}'' and ``\textit{first-order attention}''  on the real-world datasets. }\label{table:single_two_tower_full_att_k_hop_attn}
\end{table}

==> sections/tables/compare_cont_method.tex <==
\begin{table}[h]
\centering
\caption{Comparison of the \textit{Micro}- and \textit{Macro}-\textit{AUC} score of \DGT, JODIE on the real-world datasets.
% , where ``$-$'' stands for the code is not runable due to more than $24$GB GPU memory is required during training.
} \label{table:cont_method}
\scalebox{0.99}{
\begin{tabular}{llccc}
\hline\hline
\textbf{Method}                & \textbf{Metric}    & \textbf{UCI}        & \textbf{Yelp}        & \textbf{ML-10M}     \\ \hline\hline

\multirow{2}{*}{\DGT}    & \text{Micro-AUC}   & $\bm{87.91\pm0.32}$      & $\bm{ 73.39 \pm 0.21}$      & $ \bm{95.30 \pm 0.36}$     \\ % \cline{2-8} 
                         & \text{Macro-AUC}   & $\bm{88.49\pm0.43}$      & $\bm{ 74.31 \pm 0.23}$      & $ \bm{96.16 \pm 0.22}$     \\ \hline
\multirow{2}{*}{JODIE}   & \text{Micro-AUC}   & $57.99\pm0.34$           & $ 59.85 \pm 0.32 $          & $ 62.84 \pm 0.47$          \\ % \cline{2-8} 
                         & \text{Macro-AUC}   & $57.21\pm0.37$           & $61.01\pm 0.44$             & $ 61.30 \pm 0.46 $         \\ \hline
\multirow{2}{*}{TGAT}    & \text{Micro-AUC}   & $ 48.15 \pm 0.45$        & $ 51.95 \pm 0.39$           & $ 52.15 \pm 0.51$          \\ % \cline{2-8} 
                         & \text{Macro-AUC}   & $ 49.02 \pm 0.43$        & $ 52.78 \pm 0.40$           & $ 51.15 \pm 0.50$          \\ \hline\hline
\end{tabular}
}
% \vspace{-5pt}
\end{table}


==> sections/tables/compare_with_without_pretrain.tex <==
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{llcccc}
\hline
\textbf{Method}                    & \textbf{Metric}    &  \textbf{Enron}     & \textbf{UCI}        & \textbf{ML-10M} \\ \hline\hline
\multirow{2}{*}{Without pre-train} & \text{Micro-AUC}   & $84.02\pm2.98$      &    $ 86.03\pm0.89 $ & $90.12\pm0.70$ \\ % \cline{2-8} 
                                   & \text{Macro-AUC}   & $83.84\pm3.29$      &    $ 86.80\pm1.00 $ & $89.68\pm0.69$ \\ \hline
% \multirow{2}{*}{Pre-train with  $\mathcal{L}_\text{view}$}    
%                                   & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
%                                   & \text{Macro-AUC}   &                     &                     &                  \\ \hline\hline
% \multirow{2}{*}{Pre-train with  $\mathcal{L}_\text{recon}$}    
%                                   & \text{Micro-AUC}   &                     &                     &                 \\ % \cline{2-8} 
%                                   & \text{Macro-AUC}   &                     &                     &                 \\ \hline\hline
\multirow{2}{*}{With pre-train
% Pre-train with  $\mathcal{L}_\text{view}$ and $\mathcal{L}_\text{recon}$
}
                                   & \text{Micro-AUC}   & $\bm{87.32\pm0.87}$ & $\bm{87.91\pm0.60}$ & $\bm{95.81\pm0.21}$ \\ % \cline{2-8} 
                                   & \text{Macro-AUC}   & $\bm{87.84\pm0.85}$ & $\bm{88.95\pm0.53}$ & $\bm{96.16\pm0.22}$ \\ \hline
                                   
\end{tabular}
}
\vspace{-5pt}
\caption{Comparison of the \textit{Micro}- and \textit{Macro}-\textit{AUC} of \text{with} and \text{without} pre-training on the real-world datasets. }\label{table:pretrain_vs_not_pretrain}
\end{table}


==> sections/tables/config.tex <==
\begin{table}[h]
\caption{Hyper-parameters used in \DGT for different datasets. ``-'' stands for hyper-parameters that are not required.} \label{table:hyper_parameters}
\centering
\begin{tabular}{lccccccc}
\hline\hline
                                          & \textbf{Enron} & \textbf{RDS} & \textbf{UCI} & \textbf{Yelp} & \textbf{ML-10M} & \textbf{Wiki} & \textbf{Reddit} \\ \hline\hline
\text{Self-attention head}              &  $16$           & $16$           & $8$          & $8$           & $8$             & $8$                & $8$             \\ \hline
\text{Hidden dimension}                 &  $256$          & $256$          & $128$        & $128$         & $128$           & $128$              & $128$           \\ \hline
\text{Number of layer}                  &  $2$            & $2$            & $6$          & $4$           & $4$             & $2$                & $2$             \\ \hline
\text{Hidden feature dropout out ratio} &  $0.5$          & $0.5$          & $0.5$        & $0.5$         & $0.5$           & $0.5$              & $0.5$           \\ \hline
\text{Self-attention dropout ratio}     &  $0.1$          & $0.1$          & $0.1$        & $0.5$         & $0.5$           & $0.1$              & $0.1$           \\ \hline
\text{Negative sampling ratio}          &  $50$           & $10$           & $10$         & $10$          & $10$            & $-$               & $-$            \\ \hline
\text{Maximize shortest path distance}  &  $5$            & $5$            & $5$          & $5$           & $5$             & $5$                & $5$             \\ \hline
\text{Mini-batch size}                  &  $512$          & $512$          & $512$        & $512$         & $512$           & $800$              & $800$           \\ \hline\hline
\end{tabular}
\end{table}
